R2N2: Residual Recurrent Neural Networks for Multivariate Time Series Forecasting

Multivariate time-series modeling and forecasting is an important problem with numerous applications. Traditional approaches such as VAR (vector auto-regressive) models and more recent approaches such as RNNs (recurrent neural networks) are indispensable tools in modeling time-series data. In many multivariate time series modeling problems, there is usually a significant linear dependency component, for which VARs are suitable, and a nonlinear component, for which RNNs are suitable. Modeling such times series with only VAR or only RNNs can lead to poor predictive performance or complex models with large training times. In this work, we propose a hybrid model called R2N2 (Residual RNN), which first models the time series with a simple linear model (like VAR) and then models its residual errors using RNNs. R2N2s can be trained using existing algorithms for VARs and RNNs. Through an extensive empirical evaluation on two real world datasets (aviation and climate domains), we show that R2N2 is competitive, usually better than VAR or RNN, used alone. We also show that R2N2 is faster to train as compared to an RNN, while requiring less number of hidden units.

==> future.tex <==
The idea of Residual RNNs paves the way for a lot of future work, mainly in exploring different base linear models. As we mention earlier, the base model can be customized to certain special needs of the data's domain. As a specific direction we propose to explore Kalman Filters as a base model in R2N2. Another direction to take is to explore more varied datasets and analyze the performance of R2N2s on those to verify the consistency of the performance presented here.
